SEVerA: Verified Synthesis of Self-Evolving Agents

Recent advances have shown the effectiveness of self-evolving LLM agents on tasks such as program repair and scientific discovery. In this paradigm, a planner LLM synthesizes an agent program that invokes parametric models, including LLMs, which are then tuned per task to improve performance. However, existing self-evolving agent frameworks provide no formal guarantees of safety or correctness. Because such programs are often executed autonomously on unseen inputs, this lack of guarantees raises reliability and security concerns. We formulate agentic code generation as a constrained learning problem, combining hard formal specifications with soft objectives capturing task utility. We introduce Formally Guarded Generative Models (FGGM), which allow the planner LLM to specify a formal output contract for each generative model call using first-order logic. Each FGGM call wraps the underlying model in a rejection sampler with a verified fallback, ensuring every returned output satisfies the contract for any input and parameter setting. Building on FGGM, we present SEVerA (Self-Evolving Verified Agents), a three-stage framework: Search synthesizes candidate parametric programs containing FGGM calls; Verification proves correctness with respect to hard constraints for all parameter values, reducing the problem to unconstrained learning; and Learning applies scalable gradient-based optimization, including GRPO-style fine-tuning, to improve the soft objective while preserving correctness. We evaluate SEVerA on Dafny program verification, symbolic math synthesis, and policy-compliant agentic tool use ($\tau^2$-bench). Across tasks, SEVerA achieves zero constraint violations while improving performance over unconstrained and SOTA baselines, showing that formal behavioral constraints not only guarantee correctness but also steer synthesis toward higher-quality agents.

==> contents/5_proofs.tex <==
% \section{Formal Proofs}

==> contents/junk.tex <==
\begin{figure}[htbp]
\centering
% --------- Left column: built-in rules ----------
\begin{minipage}{0.45\textwidth}
\centering
\begin{prooftree}
  \AxiomC{$\evalto{\te{Inherit$(t_1, t_2)$}}{\te{$T$}}$}
  \UnaryInfC{$\abs{\te{isType(\te{$t_1$})}} \abscomp \abs{\te{isType(\te{$t_2$})}}$}
\end{prooftree}
\begin{prooftree}
  \AxiomC{$\psi_{1} = \psi_{2} \land P$}
  \UnaryInfC{$\abs{\psi_{1}} \abscomp \abs{\psi_{2}}$}
\end{prooftree}
\begin{prooftree}
  \AxiomC{$\psi_{2} = \psi_{1} \lor P$}
  \UnaryInfC{$\abs{\psi_{1}} \abscomp \abs{\psi_{2}}$}
\end{prooftree}
\begin{prooftree}
  \AxiomC{$\forall x.\; (\psi_{1}(x) \Rightarrow \psi_{2}(x))$}
  \UnaryInfC{$\abs{\psi_{1}} \abscomp \abs{\psi_{2}}$}
\end{prooftree}
\end{minipage}
% --------- Right column: user-defined rules ----------
\begin{minipage}{0.45\textwidth}
\centering
{\color{blue}
\begin{prooftree}
  \AxiomC{$T$}
  \UnaryInfC{$\abs{\text{LinExp}} \abscomp \abs{\text{PolyExpDegree}(\te{"1"})}$}
\end{prooftree}
}
{\color{blue}
\begin{prooftree}
  \AxiomC{$\text{\isType{\te{"int"}}{x}}\!\Downarrow\!T$}
  \UnaryInfC{$\abs{\text{PolyExpDegree}(x)} \abscomp \abs{\text{PolyExp}}$}
\end{prooftree}
}
{\color{blue}
\begin{prooftree}
  \AxiomC{$\isType{\te{"int"}}{{x}}\!\Downarrow\!T$}
  \AxiomC{$\isType{\te{"int"}}{y}\!\Downarrow\!T$}
  \AxiomC{$(x \le_{\text{(int)}} y)\!\Downarrow\!T$}
  \TrinaryInfC{$\abs{\text{PolyExpDegree}(x)} \abscomp \abs{\text{PolyExpDegree}(y)}$}
\end{prooftree}
}
\end{minipage}
\hfill
\caption{An example of basic proof rules (black) and user specified proof rules (blue) that enable the \Tool to infer the partial order relation between new abstract elements introduced by the Drafter LLM.}
\end{figure}

\begin{figure}
    \centering
\begin{lstlisting}[language=Dafny]
// Polynomial regression from given data list.
function PolyRegressor(data: string, d: string) returns (r: string)
  requires (*@\isType{\text{"list[tuple[real, real]]"}}{data} @*) (*@ $\bigwedge$ @*)(*@\isType{\text{"int"}}{d} @*)
  ensures PolyExpDegree(x)(r)

// Evaluates the polynomial on a given data-point.
function eval(expression: string, val: string) returns (r: string)
  requires PolyExp(expression) (*@ $\bigwedge$ @*)(*@\isType{\text{"real"}}{val} @*)
  ensures (*@\isType{\text{"real"}}{r} @*)
  
\end{lstlisting}
    \caption{Set of user defined operators and their abstract semantics which the Drafter can use for constructing the plan.}
    \label{fig:userDefinedOPs}
\end{figure}



\begin{figure}
    \centering
\begin{lstlisting}[language=Dafny]
(*@\com{// Agent Definition} @*)
function SymbolicRegression(img: string, x: string) returns (r: string)
  requires (*@\isType{\text{"image"}}{img} @*) (*@ $\bigwedge$ @*)(*@\isType{\text{"real"}}{x} @*)
  ensures  (*@\isType{\text{"real"}}{r} @*) (*@ $\bigwedge$ @*) (r (*@ $\geq_{real}$ @*) "0")
{
  var y := x (*@ $*_{real}$ @*) x; 
  return r;
}
\end{lstlisting}
    \caption{Successfully Verified Drafter plan. However, it does not uses the \te{"img"} input producing suboptimal result.}
    \label{fig:verifiedBadPlan}
\end{figure}

\begin{figure}
    \centering
\begin{lstlisting}[language=Dafny]
(*@\com{// Abstract Semantics of Drafter-introduced operators} @*)
(*@\com{// Op trainer required to find concrete implementation} @*)
(*@\com{// in accordance to abstract semantics.} @*)
function processImgData(img: string, instruction: string) returns (y: string)
  requires (*@\isType{\text{"image"}}{img} @*)
  ensures (*@\isType{\text{"list[tuple[real, real]]"}}{y} @*)
{}

(*@\com{// Agent Definition} @*)
function SymbolicRegression(img: string, x: string) returns (r: string)
  requires (*@\isType{\text{"image"}}{img} @*) (*@ $\bigwedge$ @*)(*@\isType{\text{"real"}}{x} @*)
  ensures  (*@\isType{\text{"real"}}{r} @*) (*@ $\bigwedge$ @*) (r (*@ $\geq_{real}$ @*) "0")
{
  var instruct := (*@\textcolor{dafnypurple}{"Extract (x, y) tuples from input image"};@*);
  var data := (*@ \textcolor{red}{processImgData}@*)(img, instruct); (*@\com{// Op trainer implements} @*) 
  var linExp := PolyRegressor(data, "1");
  var y := eval(linExp, x);
  (*@\setlength{\fboxsep}{0pt}\colorbox{highlightred}{\strut \color{white} return y; // Post condition does not verify}@*)
}
\end{lstlisting}
    \caption{Drafter plan with \textcolor{red}{`processImgData`} introduced as the new abstract operator. However, the post condition does get proved.}
    \label{fig:unVerifiedAttempt}
\end{figure}



\begin{figure}
    \centering
\begin{lstlisting}[language=Dafny]
(*@\com{// Abstract Semantics of Drafter-introduced operators} @*)
(*@\com{// Op trainer required to find concrete implementation} @*)
(*@\com{// in accordance to abstract semantics.} @*)
function processImgData(img: string, instruction: string) returns (y: string)
  requires (*@\isType{\text{"image"}}{img} @*)
  ensures (*@\isType{\text{"list[tuple[real, real]]"}}{y} @*)
{}

(*@\com{// Agent Definition} @*)
function SymbolicRegression(img: string, x: string) returns (r: string)
  requires (*@\isType{\text{"image"}}{img} @*) (*@ $\bigwedge$ @*)(*@\isType{\text{"real"}}{x} @*)
  ensures  (*@\isType{\text{"real"}}{r} @*) (*@ $\bigwedge$ @*) (r (*@ $\geq_{real}$ @*) "0")
{
  var instruct = (*@\textcolor{dafnypurple}{"Extract (x, sqrt(y)) tuples from input image"};@*)
  var d := (*@ \textcolor{red}{processImgData}@*)(img, instruct); (*@\com{// Op trainer implements} @*) 
  var polyExp := PolyRegressor(data, "2");
  var y := eval(polyExp, x);
  var z := y (*@$*_{real}$@*) y; (*@\com{// builtin $*_{real}$ semantics ensures z $\geq_{real}$ "0"} @*)
  return z;
}
\end{lstlisting}
    \caption{\textcolor{softgreen}{Successfully Verified} Drafter plan with \textcolor{red}{`processImgData`} introduced as the new abstract operator. Op trainers task is to implement the \textcolor{red}{`processImgData`} following the defined abstract semantics.}
    \label{fig:successFullyVerifiedAttempt}
\end{figure}


\begin{figure}
    \centering
\begin{lstlisting}[language=Dafny]
(*@\com{// Abstract Semantics of Drafter-introduced operators} @*)
(*@\com{// Op trainer required to find concrete implementation} @*)
(*@\com{// in accordance to abstract semantics.} @*)
function processImgData(img: string, instruction: string) returns (y: string)
  requires (*@\isType{\text{"image"}}{img} @*)
  ensures (*@\isType{\text{"list[tuple[real, real]]"}}{y} @*)
{
    var i := 0;
    var y;
    while i < [[(*@\textcolor{blue}{attempts}]]@*)
    // Invariant: 
    {
     y := VLLM(...);
    }
    if (\isType{\text{"list[tuple[real, real]]"}}{y}) {
     return y;
    } else {
    // A default value i.e. [] that satisfies 
    // (*@\textcolor{blue}{\isType{\text{"list[tuple[real, real]]"}}{"[]"}} @*)
     return "[]";
    }
}
\end{lstlisting}


\end{figure}

% \begin{prooftree}
%   \AxiomC{$\psi_{1} = \psi_{2} \land P$}
%   \UnaryInfC{$\psi_{1} \abscomp \psi_{2}$}
% \end{prooftree}

% \begin{prooftree}
%   \AxiomC{$\psi_{2} = \psi_{1} \lor P$}
%   \UnaryInfC{$\psi_{1} \abscomp \psi_{2}$}
% \end{prooftree}

% \begin{prooftree}
%   \AxiomC{$\forall x.\; (\psi_{1}(x) \Rightarrow \psi_{2}(x))$}
%   \UnaryInfC{$\psi_{1} \abscomp \psi_{2}$}
% \end{prooftree}

% % ------------------ User-defined rules ------------------

% {\color{blue}
% \begin{prooftree}
%   \AxiomC{$\text{isInt}(x)\!\Downarrow\!\text{True}$}
%   \AxiomC{$\text{isInt}(y)\!\Downarrow\!\text{True}$}
%   \AxiomC{$x \le_{\text{(int)}} y$}
%   \TrinaryInfC{$\text{PolyExpDegree}(x) \abscomp \text{PolyExpDegree}(y)$}
% \end{prooftree}
% }

% {\color{blue}
% \begin{prooftree}
%   \AxiomC{$\text{True}$}
%   \UnaryInfC{$\text{LinExp} \abscomp \text{PolyExpDegree}(\text{"1"})$}
% \end{prooftree}
% }
% {\color{blue}
% \begin{prooftree}
%   \AxiomC{$\text{isInt}(x)\!\Downarrow\!\text{True}$}
%   \UnaryInfC{$\text{PolyExpDegree}(x) \abscomp \text{PolyExp}$}
% \end{prooftree}
% }
\subsection{A Subsection Sample}
%
\begin{thebibliography}{8}
\bibitem{ref_article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{ref_lncs1}
Author, F., Author, S.: Title of a proceedings paper. In: Editor,
F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
Springer, Heidelberg (2016). \doi{10.10007/1234567890}

\bibitem{ref_book1}
Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
Location (1999)

\bibitem{ref_proc1}
Author, A.-B.: Contribution title. In: 9th International Proceedings
on Proceedings, pp. 1--2. Publisher, Location (2010)

\bibitem{ref_url1}
LNCS Homepage, \url{http://www.springer.com/lncs}, last accessed 2023/10/25
\end{thebibliography}

